Automated Social Science: Language Models as Scientist and Subjects

We present an approach for automatically generating and testing, in silico, social scientific hypotheses. This automation is made possible by recent advances in large language models (LLM), but the key feature of the approach is the use of structural causal models. Structural causal models provide a language to state hypotheses, a blueprint for constructing LLM-based agents, an experimental design, and a plan for data analysis. The fitted structural causal model becomes an object available for prediction or the planning of follow-on experiments. We demonstrate the approach with several scenarios: a negotiation, a bail hearing, a job interview, and an auction. In each case, causal relationships are both proposed and tested by the system, finding evidence for some and not others. We provide evidence that the insights from these simulations of social interactions are not available to the LLM purely through direct elicitation. When given its proposed structural causal model for each scenario, the LLM is good at predicting the signs of estimated effects, but it cannot reliably predict the magnitudes of those estimates. In the auction experiment, the in silico simulation results closely match the predictions of auction theory, but elicited predictions of the clearing prices from the LLM are inaccurate. However, the LLM's predictions are dramatically improved if the model can condition on the fitted structural causal model. In short, the LLM knows more than it can (immediately) tell.

==> Makefile <==
##################
# Initialization
##################
include .env

# -- Project name 
project_name  = rs
public_name = robot_scientist

# -- Timestamp
ts := $(shell /bin/date "+%Y-%m-%d---%H-%M-%S")


# -- Get and install packages
package_list.txt:
	 find ../analysis/inference/ -name *R -print0 | xargs -0 grep -h 'library*' | sed 's/library//g' | sed 's/#//g' | sed 's/ //g' | sort | uniq| sed 's/(//g' | sed 's/)//g' > package_list.txt
install_packages: package_list.txt
	cat package_list.txt | xargs -I {} Rscript -e 'install.packages("{}", repos = "http://cran.us.r-project.org")'

add_data: $(DROPBOX_PATH)/data.tar.gz
	cp $(DROPBOX_PATH)/data.tar.gz ../data/

.PHONY: check-data
check-data:
	cp $(DROPBOX_PATH)/data.tar.gz ../data/
	cd ../data && tar -xzvf data.tar.gz



#$(DROPBOX_PATH)/data.tar.gz:
#	$(error Please add data.tar.gz to the dropbox folder

# New target for extracting data
extract_data: $(DROPBOX_PATH)/data.tar.gz
	tar -xzvf $(DROPBOX_PATH)/data.tar.gz -C ../data/

##################
# Data and objects
##################


## --- 1. data 

# --- 3. List of objects
plots =
tables = 
parameters =

plots += plots/mug_love_scm.tex
plots/mug_love_scm.tex: ../analysis/inference/mug_love.py ../data/mug_love/
	cd ../analysis/inference && python mug_love.py

plots += plots/mug_love_scm_interaction.tex
plots/mug_love_scm_interaction.tex: ../analysis/inference/mug_love_interact.py ../data/mug_love/
	cd ../analysis/inference && python mug_love_interact.py

plots += plots/tax_fraud_scm.tex
plots/tax_fraud_scm.tex: ../analysis/inference/tax_fraud.py ../data/tax_fraud/
	cd ../analysis/inference && python tax_fraud.py

plots += plots/tax_fraud_scm_interaction.tex
plots/tax_fraud_scm_interaction.tex: ../analysis/inference/tax_fraud_interact.py ../data/tax_fraud/
	cd ../analysis/inference && python tax_fraud_interact.py

plots += plots/auction_art_3vars_scm.tex
plots/auction_art_3vars_scm.tex: ../analysis/inference/auction_art_3vars.py ../data/auction_art_3vars/
	cd ../analysis/inference && python auction_art_3vars.py

plots += plots/auction_art_3vars_scm_interaction.tex
plots/auction_art_3vars_scm_interaction.tex: ../analysis/inference/auction_art_3vars_interact.py ../data/auction_art_3vars/
	cd ../analysis/inference && python auction_art_3vars_interact.py

plots += plots/lawyer_interview_3var_scm.tex
plots/lawyer_interview_3var_scm.tex: ../analysis/inference/lawyer_interview_3var.py ../data/lawyer_interview_3var/
	cd ../analysis/inference && python lawyer_interview_3var.py

plots += plots/lawyer_interview_3var_scm_interaction.tex
plots/lawyer_interview_3var_scm_interaction.tex: ../analysis/inference/lawyer_interview_3var_interact.py ../data/lawyer_interview_3var/
	cd ../analysis/inference && python lawyer_interview_3var_interact.py

plots += plots/specific_prediction.pdf
plots/specific_prediction.pdf: ../analysis/prediction/panel_specific.R ../data/prediction/
	cd ../analysis/prediction && Rscript panel_specific.R

plots += plots/prediction.pdf
plots/prediction.pdf: ../analysis/prediction/panel_full.R ../data/prediction/
	cd ../analysis/prediction && Rscript panel_full.R

parameters += parameters/params.tex
parameters/params.tex: ../analysis/inference/generate_params.R ../data/lawyer_interview_3var/ ../data/tax_fraud/ ../data/auction_art_3vars/ ../data/mug_love/ ../data/misspecify_scm/
	cd ../analysis/inference && Rscript count_misspecified_scm.R && Rscript generate_params.R /analysis/inference/

## --- M.1 Makes or updates manuscript using latex & bibtext
$(project_name).pdf: $(project_name).bib $(project_name).tex $(plots) $(tables) $(parameters) 
	pdflatex -interaction=batchmode $(project_name)
	bibtex $(project_name)
	pdflatex -interaction=batchmode $(project_name)
	pdflatex -interaction=batchmode $(project_name)


dropbox: 
	cp rs.pdf ../../Dropbox/public_robot_scientist/rs.pdf


COMMENT ?= update paper

website:
	cd ../../website_benjaminmanning.io/static/files/
	git pull
	cp rs.pdf ../../website_benjaminmanning.io/static/files/rs.pdf && \
	cd ../../website_benjaminmanning.io/static/files/ && \
	git add rs.pdf && \
	git commit -m "$(COMMENT)" && \
	git push

desktop:
	cp rs.pdf ../../Desktop/rs.pdf

## --- M.2 Makes paper from scratch
clean:
	rm -f ../data/*.csv
	rm -f plots/*.png
	rm -f plots/*.tex
	rm -f plots/*.pdf
	rm -f tables/*.tex
	rm -f parameters/*.tex
	rm -f $(project_name).pdf
	rm -f $(project_name).aux
	rm -f $(project_name).bbl
	rm -f $(project_name).fls
	rm -f $(project_name).synctex.gz
	rm -f $(project_name).fdb_latexmk
	rm -f $(project_name).blg
	rm -f $(project_name).log
	rm -f $(project_name).out
	make extract_data
	make $(project_name).pdf



==> tables/auction_art_3vars_table.tex <==

\begin{table}[H]
\centering
\caption{Information automatically generated to build the SCM and design the experiment for ``3 bidders participating in an auction for a piece of art starting at fifty dollars."}
\label{tab:auction-art-3vars-table}
\
\fontsize{9pt}{10.5pt}\selectfont
\renewcommand{\arraystretch}{1.15}         

\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3cm}|p{7.5cm}|}
\hline
\multicolumn{1}{|c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{Information Name}} & \multicolumn{1}{c|}{\textbf{Information Value}} \\ \hline

\centering Final price of the piece of art (final-art-price)& \centering Measurement Question & auctioneer: what was the final bid for the piece of art at the end of the auction?  \\ \cline{2-3}
                
                        & \centering Variable Type & continuous  \\ \hline
\end{tabularx}\\
                


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Bidder 1's max budget (bid1-max-budget)
                        & \centering Attribute Treatment Values (7)  & [`\$50', `\$100', `\$150', `\$200', `\$250', `\$300', `\$350']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your maximum budget for the piece of art   \\ \cline{2-3}
                        & \centering Relevant Agent   & bidder 1   \\ \cline{2-3}
                        & \centering Variable Type & continuous  \\ \hline
\end{tabularx}\\


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Bidder 2's max budget (bid2-max-budg)
                        & \centering Attribute Treatment Values (7)  & [`\$50', `\$100', `\$150', `\$200', `\$250', `\$300', `\$350']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your maximum budget for the piece of art   \\ \cline{2-3}
                        & \centering Relevant Agent   & bidder 2   \\ \cline{2-3}
                        & \centering Variable Type & continuous  \\ \hline
\end{tabularx}\\


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Bidder 3's max budget (bid3-max-budg)
                        & \centering Attribute Treatment Values (7)  & [`\$50', `\$100', `\$150', `\$200', `\$250', `\$300', `\$350']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your maximum budget for the piece of art   \\ \cline{2-3}
                        & \centering Relevant Agent   & bidder 3   \\ \cline{2-3}
                        & \centering Variable Type & continuous  \\ \hline
\end{tabularx}\\
    \begin{minipage}{\textwidth}
    \begin{footnotesize}
      \emph{Notes: The left-most column of the table lists the variables in the SCM.
      The second column gives the name of the most important pieces of information about each variable.
      The third column shows the realized value of each piece of information named in the second column.
      The proxy attribute and one of its values are directly provided to the relevant agent in each simulation.}
    \end{footnotesize}
    \end{minipage}
\end{table}


==> tables/lawyer_interview_3var_table.tex <==

\begin{table}[H]
\centering
\caption{Information automatically generated to build the SCM and design the experiment for ``a person is interviewing for a job as a lawyer."}
\label{tab:lawyer-interview-3var-table}
\
\fontsize{9pt}{10.5pt}\selectfont
\renewcommand{\arraystretch}{1.15}         

\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3cm}|p{7.5cm}|}
\hline
\multicolumn{1}{|c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{Information Name}} & \multicolumn{1}{c|}{\textbf{Information Value}} \\ \hline

\centering Employer's Decision (hire-decision)& \centering Measurement Question & employer: have you decided to hire the job applicant?  \\ \cline{2-3}
                
                        & \centering Variable Type & binary  \\ \hline
\end{tabularx}\\
                


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Whether the applicant passed the bar exam (bar-exam-pass)
                        & \centering Attribute Treatment Values (2)  & [`not passed', `passed']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your bar exam status   \\ \cline{2-3}
                        & \centering Relevant Agent   & job applicant   \\ \cline{2-3}
                        & \centering Variable Type & binary  \\ \hline
\end{tabularx}\\


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Interviewer's level of friendliness (inter-friendly)
                        & \centering Attribute Treatment Values (5)  & [`2', `7', `12', `17', `22']   \\ \cline{2-3}
                        & \centering Proxy Attribute & number of positive phrases to use during interview   \\ \cline{2-3}
                        & \centering Relevant Agent   & employer   \\ \cline{2-3}
                        & \centering Variable Type & count  \\ \hline
\end{tabularx}\\


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Job applicant's height (job-app-height)
                        & \centering Attribute Treatment Values (8)  & [`160', `165', `170', `175', `180', `185', `190', `195']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your height in centimeters   \\ \cline{2-3}
                        & \centering Relevant Agent   & job applicant   \\ \cline{2-3}
                        & \centering Variable Type & continuous  \\ \hline
\end{tabularx}\\
    \begin{minipage}{\textwidth}
    \begin{footnotesize}
      \emph{Notes: The left-most column of the table lists the variables in the SCM.
      The second column gives the name of the most important pieces of information about each variable.
      The third column shows the realized value of each piece of information named in the second column.
      The proxy attribute and one of its values are directly provided to the relevant agent in each simulation.}
    \end{footnotesize}
    \end{minipage}
\end{table}


==> tables/mug_love_table.tex <==

\begin{table}[H]
\centering
\caption{Information automatically generated to build the SCM and design the experiment for ``two people bargaining over a mug."}
\label{tab:mug-love-table}
\
\fontsize{9pt}{10.5pt}\selectfont
\renewcommand{\arraystretch}{1.15}         

\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3cm}|p{7.5cm}|}
\hline
\multicolumn{1}{|c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{Information Name}} & \multicolumn{1}{c|}{\textbf{Information Value}} \\ \hline

\centering Whether or not a deal occurs (deal-for-mug)& \centering Measurement Question & coordinator: did the buyer and seller explicitly agree on the price of the mug during their interaction?  \\ \cline{2-3}
                
                        & \centering Variable Type & binary  \\ \hline
\end{tabularx}\\
                


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Buyer's budget (buyers-budget)
                        & \centering Attribute Treatment Values (9)  & [`3', `6', `7', `8', `10', `13', `18', `20', `25']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your budget for the mug   \\ \cline{2-3}
                        & \centering Relevant Agent   & buyer   \\ \cline{2-3}
                        & \centering Variable Type & continuous  \\ \hline
\end{tabularx}\\


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Seller's min price (sell-min-mug)
                        & \centering Attribute Treatment Values (9)  & [`3', `5', `7', `8', `10', `13', `18', `20', `25']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your minimum acceptable price for the mug   \\ \cline{2-3}
                        & \centering Relevant Agent   & seller   \\ \cline{2-3}
                        & \centering Variable Type & continuous  \\ \hline
\end{tabularx}\\


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Seller's feelings of love towards the mug (sell-love-mug)
                        & \centering Attribute Treatment Values (5)  & [`no emotional attachment', `slight emotional attachment', `moderate emotional attachment', `high emotional attachment', `extreme emotional attachment']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your emotional attachment to the mug   \\ \cline{2-3}
                        & \centering Relevant Agent   & seller   \\ \cline{2-3}
                        & \centering Variable Type & ordinal  \\ \hline
\end{tabularx}\\
    \begin{minipage}{\textwidth}
    \begin{footnotesize}
      \emph{Notes: The left-most column of the table lists the variables in the SCM.
      The second column gives the name of the most important pieces of information about each variable.
      The third column shows the realized value of each piece of information named in the second column.
      The proxy attribute and one of its values are directly provided to the relevant agent in each simulation.}
    \end{footnotesize}
    \end{minipage}
\end{table}


==> tables/tax_fraud_table.tex <==

\begin{table}[H]
\centering
\caption{Information automatically generated to build the SCM and design the experiment for ``a judge is setting bail for a criminal defendant who committed 50,000 dollars in tax fraud."}
\label{tab:tax-fraud-table}
\
\fontsize{9pt}{10.5pt}\selectfont
\renewcommand{\arraystretch}{1.15}         

\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3cm}|p{7.5cm}|}
\hline
\multicolumn{1}{|c|}{\textbf{Variable}} & \multicolumn{1}{c|}{\textbf{Information Name}} & \multicolumn{1}{c|}{\textbf{Information Value}} \\ \hline

\centering Bail amount set by the judge (bail-amt)& \centering Measurement Question & judge: what was the bail amount you set for the defendant?  \\ \cline{2-3}
                
                        & \centering Variable Type & continuous  \\ \hline
\end{tabularx}\\
                


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Defendant's criminal history (def-crim-hist)
                        & \centering Attribute Treatment Values (7)  & [`0', `1', `2', `3', `6', `9', `12']   \\ \cline{2-3}
                        & \centering Proxy Attribute & number of your prior convictions   \\ \cline{2-3}
                        & \centering Relevant Agent   & defendant   \\ \cline{2-3}
                        & \centering Variable Type & count  \\ \hline
\end{tabularx}\\


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Prior case count for judge that day (num-judge-cases)
                        & \centering Attribute Treatment Values (7)  & [`0', `2', `5', `9', `12', `18', `23']   \\ \cline{2-3}
                        & \centering Proxy Attribute & number of cases you have already heard today   \\ \cline{2-3}
                        & \centering Relevant Agent   & judge   \\ \cline{2-3}
                        & \centering Variable Type & count  \\ \hline
\end{tabularx}\\


\begin{tabularx}{\textwidth}{|p{3.25cm}|p{3.025cm}|p{7.5cm}|}
\hline
\centering Defendant's level of remorse (def-remorse)
                        & \centering Attribute Treatment Values (5)  & [`no expressed remorse', `low expressed remorse', `moderate expressed remorse', `high expressed remorse', `extreme expressed remorse']   \\ \cline{2-3}
                        & \centering Proxy Attribute & your level of expressed remorse   \\ \cline{2-3}
                        & \centering Relevant Agent   & defendant   \\ \cline{2-3}
                        & \centering Variable Type & ordinal  \\ \hline
\end{tabularx}\\
    \begin{minipage}{\textwidth}
    \begin{footnotesize}
      \emph{Notes: The left-most column of the table lists the variables in the SCM.
      The second column gives the name of the most important pieces of information about each variable.
      The third column shows the realized value of each piece of information named in the second column.
      The proxy attribute and one of its values are directly provided to the relevant agent in each simulation.}
    \end{footnotesize}
    \end{minipage}
\end{table}

